Clustering evolving data using kernel-based methods

In this thesis, we propose several modelling strategies to tackle evolving data in different contexts. In the framework of static clustering, we start by introducing a soft kernel spectral clustering (SKSC) algorithm, which can better deal with overlapping clusters with respect to kernel spectral clustering (KSC) and provides more interpretable outcomes. Afterwards, a whole strategy based upon KSC for community detection of static networks is proposed, where the extraction of a high quality training sub-graph, the choice of the kernel function, the model selection and the applicability to large-scale data are key aspects. This paves the way for the development of a novel clustering algorithm for the analysis of evolving networks called kernel spectral clustering with memory effect (MKSC), where the temporal smoothness between clustering results in successive time steps is incorporated at the level of the primal optimization problem, by properly modifying the KSC formulation. Later on, an application of KSC to fault detection of an industrial machine is presented. Here, a smart pre-processing of the data by means of a proper windowing operation is necessary to catch the ongoing degradation process affecting the machine. In this way, in a genuinely unsupervised manner, it is possible to raise an early warning when necessary, in an online fashion. Finally, we propose a new algorithm called incremental kernel spectral clustering (IKSC) for online learning of non-stationary data. This ambitious challenge is faced by taking advantage of the out-of-sample property of kernel spectral clustering (KSC) to adapt the initial model, in order to tackle merging, splitting or drifting of clusters across time. Real-world applications considered in this thesis include image segmentation, time-series clustering, community detection of static and evolving networks.

==> README <==
LaTeX bundle adjustbox
=========================
Copyright (c) 2011-2012 by Martin Scharrer <martin@scharrer-online.de>  
WWW: <https://bitbucket.org/martin_scharrer/adjustbox> (incl. bug tracker)

This bundle contains the the adjustbox package and its auxiliary packages trimclip and adjcalc.
The initial purpose of adjustbox was to supplement the standard graphics/x package, 
which defines the macros \resizebox, \scalebox and \rotatebox, with the macros \trimbox and \clipbox.
An additional \marginbox macro is also provided.
These macros are now placed in the dedicated package trimclip which is loaded by adjustbox.
The package comes with clipping driver files are provided for pdftex (incl. LuaLaTeX), dvips and xetex. A
fall-back driver which uses the pgf package is still included. 
The driver files got written by Joseph Wright (LaTeX3 project) and the package author.

The main feature of adjustbox is the general \adjustbox macro which extends the key=value
interface of \includegraphics from the graphicx package, and applies it to general text
content. It also provides further text/box modifications keys, macros and envionments.

Both adjustbox and trimclip use the adjcalc package to allow for algebraic expressions for all length
arguments. The adjcalc package can use either e-TeX, the calc package or the pgfmath package.

All macros use the authors other package collectbox to read the content as box and not as
macro argument. This allows for all forms of content including special material like verbatim content.
A special feature of collectbox is used to provide matching environments with the identical names as the
macros.



==> chapters/abbreviations/abbreviations.tex <==
\chapter{Abbreviations}
\label{ch:abbreviations}

\begin{center}
\begin{tabular}{p{.28\textwidth}p{.64\textwidth}}                                   
AMS & Average Membership Strength\\  
ARI & Adjusted Rand Index\\
BLF & Balanced Line Fit\\
$\textrm{BLF}_{\textrm{Mem}}$ & Smoothed Balanced Line Fit\\
$\textrm{Cond}$ & Conductance\\
$\textrm{Cond}_{\textrm{Mem}}$ & Smoothed Conductance\\
EF  & Expansion Factor\\ 
ESC  & Evolutionary Spectral Clustering\\ 
IKSC  & Incremental Kernel Spectral Clustering\\
IKM  & Incremental K-means\\
KKT  & Karush-Kuhn-Tucker\\
KM  & K-means\\
KSC  & Kernel Spectral Clustering\\
LFR & Benchmark graphs for testing community detection algorithms\\
LOUV  & Louvain Method\\
LS-SVM  & Least Squares Support Vector Machine\\
MKSC  & Kernel Spectral Clustering with Memory effect\\
$\textrm{Mod}$  &  Modularity\\
$\textrm{Mod}_{\textrm{Mem}}$  & Smoothed Modularity\\
NMI  & Normalized Mutual Information\\
PCA  & Principal Component Analysis\\
RBF  & Radial Basis Function\\ 
SKSC  & Soft Kernel Spectral Clustering\\
SC  & Spectral Clustering\\
SVM  & Support Vector Machine\\ 
\end{tabular}
\end{center}









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/abstract/abstract.tex <==
\chapter{Abstract}                                 
\label{ch:abstract}
Thanks to recent developments of Information Technologies, there is a profusion of available data in a wide range of application domains ranging from science and engineering to biology and business. For this reason, the demand for real-time data processing, mining and analysis is experiencing an explosive growth in recent years. Since labels are usually not available and in general a full understanding of the data is missing, clustering plays a major role in shedding an initial light. In this context, elements such as generalization to out-of-sample data, model selection criteria, consistency of the clustering results over time and scalability to large data become key issues. A successful modelling framework is offered by Least Squares Support Vector Machine (LS-SVM), which is designed in a primal-dual optimization setting. The latter allows extensions of the core models by adding additional constraints to the primal problem, by changing the objective function or by introducing new model selection criteria. In this thesis, we propose several modelling strategies to tackle evolving data in different contexts. In the framework of static clustering, we start by introducing a soft kernel spectral clustering (SKSC) algorithm, which can better deal with overlapping clusters with respect to kernel spectral clustering (KSC) and provides more interpretable outcomes. Afterwards, a whole strategy based upon KSC for community detection of static networks is proposed, where the extraction of a high quality training sub-graph, the choice of the kernel function, the model selection and the applicability to large-scale data are key aspects. This paves the way for the development of a novel clustering algorithm for the analysis of evolving networks called kernel spectral clustering with memory effect (MKSC), where the temporal smoothness between clustering results in successive time steps is incorporated at the level of the primal optimization problem, by properly modifying the KSC formulation. Later on, an application of KSC to fault detection of an industrial machine is presented. Here, a smart pre-processing of the data by means of a proper windowing operation is necessary to catch the ongoing degradation process affecting the machine. In this way, in a genuinely unsupervised manner, it is possible to raise an early warning when necessary, in an online fashion. Finally, we propose a new algorithm called incremental kernel spectral clustering (IKSC) for online learning of non-stationary data. This ambitious challenge is faced by taking advantage of the out-of-sample property of kernel spectral clustering (KSC) to adapt the initial model, in order to tackle merging, splitting or drifting of clusters across time. Real-world applications considered in this thesis include image segmentation, time-series clustering, community detection of static and evolving networks. 
                   
    
   






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/biography/biography.tex <==
\chapter*{Biography}
%\label{ch:biography}

%\ldots
%\instructionsconclusions

Rocco Langone was born in Potenza (Italy) in 1983, where he spent his high school years. In
2002 he moved to Rome to study Physics at Sapienza University of Rome. In 2005 he
received a Bachelor's degree in Physics and Information Technology. In March 2008 he
obtained the Master's degree in Physics with the thesis: \textit{A neural network model for studying the attribution of global circulation atmospheric patterns on the climate at a local scale}. Until September 2008 he worked as researcher at the National Research Council (CNR) in
Rome. He received a second Master's degree in Scientific Computing in April 2010, with the thesis: \textit{Stochastic Volatility models for European calls option pricing}. He is currently a doctoral student in machine learning, at the STADIUS research division of the Department of Electrical Engineering (ESAT) of the KU Leuven, under the supervision of prof. Johan A. K. Suykens. During his Phd Rocco served as teaching assistant for the course \textit{Artificial Neural Networks}, included in the master in Artificial Intelligence organized by the KU Leuven. He has also been involved in the \textit{Prognostic for Optimal Maintenance} projects \textit{POM 1 and POM 2}, and as member of the \textit{Optimization in Engineering Center (OPTEC)} of the KU Leuven he actively participated in the meetings and workshops and he also took part in the DYSCO study days. Rocco's scientific interests include kernel methods, neural networks, optimization, unsupervised learning (clustering and community detection), time-series analysis, big data, climate, finance, fault detection.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/nomenclaturechapter/nomenclaturechapter.tex <==
\chapter{Notation}
\label{ch:symbols}

\begin{center}
\begin{tabular}{p{.28\textwidth}p{.70\textwidth}}                                   
$x^T$ & Transpose of a vector $x$\\
$\Omega^T$ & Transpose of a matrix $\Omega$\\
$\Omega_{ij}$ & $ij$-th entry of the matrix $\Omega$\\
$I_N$ & $N \times N$ Identity matrix\\
$1_N$ & $N \times 1$ Vector of ones\\
$\mathcal{D}_{\textrm{Tr}} = \{x_i\}_{i=1}^{N_{\textrm{Tr}}}$ & Training sample of $N_{\textrm{Tr}}$ data points\\
$\varphi(\cdot)$ & Feature map\\
$\mathcal{F}$ & Feature space of dimension $d_h$\\
$K(x_i,x_j)$ & Kernel function evaluated on data points $x_i$, $x_j$\\
$\{\mathcal{A}_p\}_{p=1}^k$ & Partition composed of $k$ clusters\\
$\alpha_i^{(l)} \in \mathbb{R}$ & $i$-th entry of the dual solution vector $\alpha^{(l)}\in \mathbb{R}^{N_{\textrm{Tr}}}$\\
$D$ & $N \times N$ graph degree matrix\\   
$\mathcal{G = (V,E)}$ & Set of $N$ vertices $\mathcal{V}= \{v_i\}_{i=1}^N$ and $m$ edges $\mathcal{E}$ of a graph\\
$\mathcal{S}=\{(\mathcal{V}_t,\mathcal{E}_t)\}_{t=1}^T$ & Sequence of networks over time $T$\\ 
$\vert \cdot \vert$ & Cardinality of a set  
\end{tabular}
\end{center}












%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/preface/preface.tex <==
\chapter*{Preface}                                  

\textit{The work presented in this thesis is related to the research carried out during my doctoral studies at the STADIUS (ex SISTA) research group, inspired by the magnificent view of the Arenberg castle. It has been a priceless time full of enriching experiences both at a professional and a personal level.\\First of all, I wish to thank my promotor Johan Suykens, who about 4 years ago believed in my abilities and gave me the opportunity to start constructing my future. During the Phd, he gave me continuous support and was always prodigal of suggestions. Many thanks also to the jury members of this thesis, who accepted to review the dissertation and provided valuable comments. I would like to acknowledge my actual and former colleagues and friends at ESAT for their helpfulness regarding work issues, the free time spent together in Leuven, the spare time enjoyed after national and international conferences. Many thanks to the Erasmus students, visiting doctoral students and all the friends I met during these years. I will always remember the nice moments shared at the occasion of lunches, dinners, trips, parties etc. Many acknowledgements to my family for cheering me up in difficult times and sharing my joy in happy moments. Finally, my most special thanks go to my girlfriend Bruna, who around 2 years ago swept away the shadow surrounding my heart with love, sweetness, and empathy...}   

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/publications/publications.tex <==
\chapter*{Publications by the Author}
\label{ch:publications}

%\begin{figure}[htbp]
%\centering
%\includegraphics[width=4in]{rocco_citations.eps}
%\caption{\textbf{Citations to my articles.}}
%\label{fig:publications}
%\end{figure}

\section*{Journal papers} 

\section*{2009}
\begin{enumerate}
\item {\sc A. Pasini, G. Szpunar, G. Amori, R. Langone, M. Cristaldi}
\newblock Assessing Climatic Influences on Rodent Density-A Neural Network Modelling Approach and a Case Study in Central Italy. \em Asia-Pacific Journal of Atmospheric Sciences (2009), 45, 319-330.
%\newblock {\em Asia-Pacific Journal of Atmospheric Sciences\/} (2009), 45, 319-330.
\end{enumerate}

\section*{2010}
\begin{enumerate}
\item {\sc A. Pasini, R. Langone}
\newblock Attribution of precipitation changes on a regional scale by neural network modelling: A case study.
\newblock {\em Water\/} (2010), 2, 3, 321--332.
\item {\sc A. Pasini, R. Langone, F. Maimone, V. Pelino}
\newblock Energy-based predictions in Lorenz system by a unified formalism and neural network modelling.
\newblock {\em Nonlinear Processes in Geophysics\/} (2010), 17, 809--815.
\end{enumerate}

\section*{2012}
\begin{enumerate}
\item {\sc A. Pasini, R. Langone}
\newblock Influence of Circulation Patterns on Temperature Behavior at the Regional Scale: A Case Study Investigated via Neural Network Modelling.
\newblock {\em Journal of Climate\/} (2012),  25, 2123--2128. 
\end{enumerate}

\section*{2013}
\begin{enumerate}
\item {\sc R. Langone, C. Alzate, J. A. K. Suykens}
\newblock Kernel spectral clustering with memory effect.
\newblock {\em Physica A: Statistical Mechanics and its Applications}, (2013), 10, 2588--2606.
\item {\sc R. Mall, R. Langone, J. A. K. Suykens}
\newblock FURS: Fast and unique representative subset selection retaining large
  scale community structure.
\newblock {\em Social Network Analysis and Mining} (2013), 3, 4, 1--21.
\item {\sc R. Mall, R. Langone, J. A. K. Suykens}
\newblock Kernel spectral clustering for big data networks.
\newblock {\em Entropy 15 (Special Issue on Big Data)} (2013), 5, 1567--1586.
\end{enumerate}

\section*{2014}
\begin{enumerate}
\item {\sc R. Langone, O. M. Agudelo, B. De~Moor, J. A. K. Suykens}
\newblock Incremental kernel spectral clustering for online learning of non-stationary data.
\newblock {\em Neurocomputing\/} (2014), 139, 246-260.
\item {\sc R. Mall, R. Langone, J. A. K. Suykens}
\newblock Multilevel Hierarchical Kernel Spectral Clustering for Real-Life Large Scale Complex Networks.
\newblock {\em {PLOS ONE}} (2014), in press.
\end{enumerate}




\section*{Conference proceedings}

\subsection*{2007}
\begin{enumerate}
\item {\sc A. Pasini, G. Szpunar, G. Amori, R. Langone, M. Cristaldi}
\newblock Meteo-Climatic influences on rodent density in central Italy: a nonlinear modelling approach.
\newblock In {\em {The 6th European Conference on Ecological Modelling, ECEM'07}\/} Trieste, Italy, 27-30 November 2007. 
\end{enumerate}

\subsection*{2009}
\begin{enumerate}
\item {\sc A. Pasini, R. Langone}
\newblock Major Influences of Circulation Patterns on Temperatures in the Italian Side of the Greater Alpine Region: an Investigation via Neural Network Modelling.
\newblock In {\em {21th Conference on Climate Variability and Change, Seventh Conference on Artificial Intelligence and its Applications to the Environmental Sciences}\/} (2009), Phoenix, Arizona.
\end{enumerate}

\subsection*{2011}
\begin{enumerate}
\item {\sc R. Langone, C. Alzate, J. A. K. Suykens}
\newblock Modularity-based model selection for kernel spectral clustering.
\newblock In {\em {Proc. of the International Joint Conference on Neural
  Networks (IJCNN)}\/} (2011), 1849--1856.
\end{enumerate}

\subsection*{2012}
\begin{enumerate}
\item {\sc R. Langone, C. Alzate, J. A. K. Suykens}
\newblock Kernel spectral clustering for community detection in complex  networks.
\newblock In {\em {Proc. of the International Joint Conference on Neural
  Networks IJCNN}\/} (2012), 2596--2603.
\item {\sc R. Langone, J. A. K. Suykens}
\newblock Community detection using kernel spectral clustering with memory.
\newblock {\em Journal of Physics: Conference Series 410} (2013), 1, 012100.  
    
\end{enumerate}  

\subsection*{2013}
\begin{enumerate}
\item {\sc R. Langone, R. Mall, J. A. K. Suykens}
\newblock Soft kernel spectral clustering.
\newblock In {\em Proc. of the International Joint Conference on Neural
  Networks (IJCNN)\/} (2013), 1028--1035.
\item {\sc R. Langone, C. Alzate, B. De~Ketelaere, J. A. K. Suykens}
\newblock {Kernel spectral clustering for predicting maintenance of industrial
  machines}.
\newblock In {\em IEEE Symposium Series on Computational Intelligence (SSCI)\/} (2013), 39--45. 
\item {\sc R. Mall, R. Langone, J. A. K. Suykens}
\newblock {Highly Sparse Reductions to Kernel Spectral Clustering}.
\newblock In {\em 5th International Conference on Pattern Recognition and
  Machine Intelligence\/} (2013), 163--169.  
\item {\sc R. Mall, R. Langone, J. A. K. Suykens}
\newblock {Self-Tuned Kernel Spectral Clustering for Large Scale Networks}.
\newblock In {\em IEEE International Conference on Big Data \/} (2013), Santa Clara (USA).  
\item {\sc D. Peluffo, S. Garcia, R. Langone, J. A. K. Suykens, G. Castellanos}
\newblock Kernel spectral clustering for dynamic data using multiple kernel
  learning.
\newblock In {\em Proc. of the International Joint Conference on Neural
  Networks (IJCNN)\/} (2013), 1085--1090.
\end{enumerate}  

\subsection*{2014}
\begin{enumerate}
\item {\sc R. Mall, R. Langone, J. A. K. Suykens}
\newblock {Agglomerative Hierarchical Kernel Spectral Clustering for Large Scale Networks}.
\newblock In {\em  ESANN, Special Session: Learning and Modelling Big Data.\/} (2014).  
\item {\sc R. Mall, S. Mehrkanoon, R. Langone, J. A. K. Suykens}
\newblock Optimal Reduced Sets for Sparse Kernel Spectral Clustering.
\newblock In {\em {Proc. of the International Joint Conference on Neural
  Networks (IJCNN)}\/} (2014), in press.
\end{enumerate}

\section*{Abstracts}

\subsection*{2007}
\begin{enumerate}
\item {\sc G. Szpunar, G. Amori, A. Pasini, R. Langone, M. Cristaldi}
\newblock Rodent density and climate in Central Italy: a modelling approach.
\newblock In {\em { 14th Int. Symp. On Environmental Pollution and its impact on Life in the Mediterranean Region}\/}, Sevilla, 2007. 
\end{enumerate}

\subsection*{2011}
\begin{enumerate}
\item {\sc R. Langone, J. A. K. Suykens}
\newblock {Community detection via kernel-based methods}.
\newblock In {\em DYSCO Study Day.\/} November 29, 2011.
\item {\sc R. Langone, J. A. K. Suykens}
\newblock {Kernel-based methods for optimal maintenance of industrial machines}.
\newblock In {\em Predictive maintenance in industry, final \uppercase{pom} workshop.\/} March 30, 2011, Gent (Belgium).  
\end{enumerate}


\subsection*{2012}
\begin{enumerate}
\item {\sc R. Langone, J. A. K. Suykens}
\newblock {Community detection via kernel spectral clustering}.
\newblock In {\em 31st Benelux meeting on Systems and Controls.\/} March 27-29, 2012. 
\item {\sc R. Langone, J. A. K. Suykens}
\newblock {Kernel spectral clustering (software demo)}.
\newblock In {\em OPTEC retreat WG2 Meeting.\/} November 9, 2012.
\end{enumerate}


\subsection*{2013}
\begin{enumerate}
\item {\sc R. Langone, J. A. K. Suykens}
\newblock {Incremental Kernel Spectral Clustering}.
\newblock In {\em International Conference on Mathematical Modelling in Physical
Sciences (IC-MSQUARE)\/} (2013),  Prague, Czech Republic.
\end{enumerate}

\subsection*{2014}
\begin{enumerate}
\item {\sc B. Piccart, R. Langone}
\newblock {Prediction of remaining useful lifetime of industrial machinery}.
\newblock In {\em Innovative solutions for predictive maintenance and performance optimization in industry, final workshop \uppercase{pom}2 project\/} (2014), March 25, Leuven.
\item {\sc R. Langone, R. Mall, J. A. K. Suykens}
\newblock {Clustering data over time using kernel spectral clustering with memory}.
\newblock In {\em DYSCO Study Day.\/} May 16, 2014.
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}



==> defs.tex <==
% Some useful packages
\usepackage{amssymb,amsthm}
\usepackage{amsmath}

% useful: TODO notes
\usepackage{todonotes}
%fix placement of todo notes (see todonotes manual)
\setlength{\marginparwidth}{(\stockwidth-\columnwidth)/2-.35cm}

% Some nice colors
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\cyan}[1]{\textcolor{cyan}{#1}}
\newcommand{\magenta}[1]{\textcolor{magenta}{#1}}
\newcommand{\yellow}[1]{\textcolor{yellow}{#1}}
\newcommand{\orange}[1]{\textcolor{orange}{#1}}
\newcommand{\violet}[1]{\textcolor{violet}{#1}}
\newcommand{\purple}[1]{\textcolor{purple}{#1}}
\newcommand{\brown}[1]{\textcolor{brown}{#1}}
\newcommand{\gray}[1]{\textcolor{gray}{#1}}
\newcommand{\darkgray}[1]{\textcolor{darkgray}{#1}}
\newcommand{\lightgray}[1]{\textcolor{lightgray}{#1}}
\newcommand{\bred}[1]{\textbf{\textcolor{red}{#1}}}


\usepackage[backref=false]{hyperref} %ho aggiunto io

==> mycoverpage.tex <==
% Redefine in this file the commands to generate the front and back cover:
%
%   \makefrontcovergeneral{xskip}{clearpage}
%   \makebackcovergeneral{xskip}{clearpage}
%
% You can start from their definition in adsphd.cls. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% My own cover page
\makeatletter

%% \renewcommand{\makefrontcovergeneral}[2]{%
%%   %
%%   % Create header
%%   \frontcoverheader{#1}
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Title, subtitle, authorname, text and date can be moved around.
%%   % Change the textblock* commands below. 
%%   %
%%   % Syntax of textblock environment:
%%   % 
%%   %   \begin{textblock*}{width}(xpos,ypos)
%%   %     ...
%%   %   \end{textblock*}
%%   % 
%%   % !! Make sure not to remove the '+#1' part!!!
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Place the title
%%   \begin{textblock*}{120mm}(17.5mm+#1,89.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \raggedright\selectfont\LARGE\sffamily\textbf{\@title}
%%   \end{textblock*}
%%   %
%%   % Place the subtitle
%%   \begin{textblock*}{120mm}(17.5mm+#1,92.0mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \Large\sffamily{\@subtitle}
%%   \end{textblock*}
%%   %
%%   % Place the author name
%%   \begin{textblock*}{120mm}(17.5mm+#1,109.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \Large\sffamily\@authorf\ \MakeUppercase\@authorl
%%   \end{textblock*}
%%   %
%%   %\begin{textblock}{120}(0,115)
%%   \begin{textblock*}{120mm}(17.5mm+#1,132.0mm)
%%   \textblockcolour{}
%%   \includegraphics*{image/coverfigure}
%%   \end{textblock*}
%%   %
%%   % Place the misc text
%%   \begin{textblock*}{60mm}(96.5mm+#1,187.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   {\small\sffamily Dissertation presented in partial\\
%%   fulfillment of the requirements for\\
%%   the degree of Doctor\\
%%   in \@degree}
%%   \end{textblock*}
%%   %
%%   % Place date
%%   \begin{textblock*}{160mm}(0mm+#1,221.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \begin{center} {\small\sffamily\@date }\end{center}
%%   \end{textblock*}
%%   
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Add footer
%%   \frontcoverfooter{#2}
%% 
%% }

\makeatother

